Adventures in Monitorability: From Branching to Linear Time and Back Again

This paper establishes a comprehensive theory of runtime monitorability for Hennessy-Milner logic with recursion, a very expressive variant of the modal $\mu$-calculus. It investigates the monitorability of that logic with a linear-time semantics and then compares the obtained results with ones that were previously presented in the literature for a branching-time setting. Our work establishes an expressiveness hierarchy of monitorable fragments of Hennessy-Milner logic with recursion in a linear-time setting and exactly identifies what kinds of guarantees can be given using runtime monitors for each fragment in the hierarchy. Each fragment is shown to be complete, in the sense that it can express all properties that can be monitored under the corresponding guarantees. The study is carried out using a principled approach to monitoring that connects the semantics of the logic and the operational semantics of monitors. The proposed framework supports the automatic, compositional synthesis of correct monitors from monitorable properties.

==> alternative.tex <==
% !TEX root = main.tex

\begin{figure}[!h]
  \textbf{Satisfaction Semantics}
\begin{align*}
  &\sat{\epsilon}{\hTru} \\
  &\sat{\ftV}{\hOr{\hV_1}{\hV_2}} && \text{ if } \sat{\ftV}{\hV_1}  \text{ or } \sat{\ftV}{\hV_2}\\
  &\sat{\ftV}{\hAnd{\hV_1}{\hV_2}} && \text{ if } \sat{\ftV}{\hV_1}  \text{ and } \sat{\ftV}{\hV_2}\\
  &\sat{\acta\ftV}{\hSuf{\ASet}{\hV}} && \text{ if } \acta \in \ASet \text{ and } \sat{\ftV}{\hV}\\
  &\sat{\acta\ftV}{\hNec{\ASet}{\hV}} &&  \acta \not\in \ASet \text{ or } \vsat{\ftV}{\hV}\\
  % \text{ if } \acta \in \ASet \text{ implies } \sat{\ftV}{\hV}\\
  &\sat{\ftV}{\hMinX{\hV}} && \text{ if } \sat{\ftV}{\hV\subC{\hMinX{\hV}}{\hVarX}}
\end{align*}
\textbf{Violation Semantics}
\begin{align*}
  &\vsat{\epsilon}{\hFls} \\
  &\vsat{\ftV}{\hOr{\hV_1}{\hV_2}} && \text{ if } \vsat{\ftV}{\hV_1}  \text{ and } \vsat{\ftV}{\hV_2}\\
  &\vsat{\ftV}{\hAnd{\hV_1}{\hV_2}} && \text{ if } \vsat{\ftV}{\hV_1}  \text{ or } \vsat{\ftV}{\hV_2}\\
  &\vsat{\acta\ftV}{\hSuf{\ASet}{\hV}} && \text{ if } \acta \not\in \ASet \text{ or } \vsat{\ftV}{\hV}\\
  &\vsat{\acta\ftV}{\hNec{\ASet}{\hV}} && \text{ if } \acta \in \ASet \text{ and }  \vsat{\ftV}{\hV}\\
  &\vsat{\ftV}{\hMaxX{\hV}} && \text{ if } \vsat{\ftV}{\hV\subC{\hMaxX{\hV}}{\hVarX}}
\end{align*}
\caption{\UHML  Linear-Time Prefix Satisfaction and Violation Semantics}
\label{fig:recHML-sat-vio}
\end{figure}


\begin{thm}[Alternative Semantics]
  % [Prefix Satisfaction and Violation Semantics Characterisation]
  % \qquad
  % \begin{description}
  %   \item[Soundness:]
    \sat{\ftV}{\hV} \text{ iff } $\forall \tV \cdot \ftV\tV \in \hSem{\hV}$ \quad \text{and} \quad \vsat{\ftV}{\hV} \text{ iff } $\forall \tV \cdot \ftV\tV \not\in \hSem{\hV}$
  %   \item[Completeness:] \sat{\ftV}{\hV} implies $\forall \tV \cdot \ftV\tV \in \hSemL{\hV}$ \quad and \quad \vsat{\ftV}{\hV} implies $\forall \tV \cdot \ftV\tV \not\in \hSemL{\hV}$
  % \end{description}
\end{thm}
\begin{proof}
  \af{ToDo}
\end{proof}


==> bounded.tex <==
% !TEX root = main.tex


As we saw, in the context of finfinite traces we lose full completeness for monitors.
For example, $\hNec{\act}{\hNec{\act}\hFls}$ is not complete-monitorable, because after seeing $\act$, even if $\act$ is not observed again,
a monitor cannot know that. Of course, the situation would be different if the monitor could receive information about the termination of the process, or other static information. This situation is examined in \cite{AceAFI:18:FOSSACS}.
However, even without such extensions of the framework, we can see a way for the monitor to reach a proper conclusion for that formula.
For instance, in the case of $\hNec{\act}{\hNec{\act}\hFls}$, if we see at least two actions, then we can safely reach a conclusion about the satisfaction or violation of the formula.
We can generalize this to the notion of $k$-complete monitors, that are complete for a formula, as long as they are guaranteed to observe a certain number of events.


\begin{defn}
We say that monitor $\mV$ is 
$k$-complete for a formula $\hV$ when 
$\mV$ is complete for $\hV$ over finfinite traces of length at least $k$.
% 
% for every trace $t$ of length at least $k$, $t \notin \hmeaning{\hV}$ implies that $\mV$ rejects $t$. Similarly, we can define that $\mV$ is $k$-complete and $k$-complete for $\hV$.
We say that $\mV$ is finitely complete for $\hV$ is there is a positive integer $k$, such that $\mV$ is $k$-complete for  $\hV$.
\end{defn}

\begin{lem}
If $\hV$ has modal depth $d$, then $m(\hV)$ is sound and $d$-complete for $\hV$.
\end{lem}

\begin{proof}
By Proposition \ref{prop:hml-monitorable}, $\hSyn{\hV}$ is sound for $\hV$. 
That $\hSyn{\hV}$ is $d$-complete for $\hV$ follows by a straightforward induction on $\hV$.
\end{proof}


==> randomA.tex <==
% !TEX root = main.tex

%\ac{to use wherever it fits:}

\begin{rem}
\Cref{thm:stronger-HML-maximality}
demonstrates that \HML can express any property of infinite traces that has a complete monitor in any monitoring system, assuming that verdicts remain irrevocable.
%
Unfortunately, this result cannot be replicated for partial completeness.
For instance, let $L \subseteq (\Act \setminus \{ e \})^*$ be a non-regular language, where $e \in \Act$ is a special symbol, and $Le = \{ we\tV \mid w \in L \text{ and } \tV \in \Act^\omega \}$.
If $Le$ could be expressed in $\CHML$, then there would be a monitor for $Le$, and by a straightforward use of \Cref{prop:monitor2automaton}, we could construct a finite automaton that recognizes $L$, which is a contradiction.
Yet, we could imagine appropriate choices for $L$ and monitoring systems in which $Le$ is monitorable.
These can range from computationally demanding ones, such as an encoding of the Halting Problem and Turing Machines that read until $e$, to more reasonable ones, such as a context-free language and monitors with some kind of memory.
\end{rem}


==> randomK.tex <==
% !TEX root = main.tex


